DESI Strong Lens Foundry I: HST Observations and Modeling with GIGA-Lens

We present the Dark Energy Spectroscopic Instrument (DESI) Strong Lens Foundry. We discovered $\sim 3500$ new strong gravitational lens candidates in the DESI Legacy Imaging Surveys using residual neural networks (ResNet). We observed a subset (51) of our candidates using the Hubble Space Telescope (HST). All of them were confirmed to be strong lenses. We also briefly describe spectroscopic follow-up observations by DESI and Keck NIRES programs. From this very rich dataset, a number of studies will be carried out, including evaluating the quality of the ResNet search candidates and lens modeling. In this paper, we present our initial effort in these directions. In particular, as a demonstration, we present the lens model for DESI-165.4754-06.0423, with imaging data from HST, and lens and source redshifts from DESI and Keck NIRES, respectively. In this effort, we have applied a \emph{fully} forward-modeling Bayesian approach (GIGA-Lens), using \emph{multiple} GPUs, for the first time in both regards, to a strong lens with HST data, or any high resolution imaging.

==> physical_model.tex <==
The EPL model is characterized by the surface mass density expressed in units of the critical density, commonly referred to as convergence,
\begin{equation}
    \kappa(x_{lens}, y_{lens}) = \frac{3-\gamma}{2}\left(\frac{\theta_E}{\sqrt{q x_{lens}^2+y_{lens}^2 / q}}\right)^{\gamma-1},
\end{equation}
where $\theta_E$ is the Einstein radius, $\gamma$ is the mass profile slope, $(x_{lens}, y_{lens})$ are lens-centric coordinates, and $q$ is the axial ratio. 
The deflection angle can be calculated iteratively using the Gaussian hypergeometric function, reaching a truncation error $\lesssim 10^{-16}$ within $35$ iterations for $q\gtrsim 0.5$ \citep{tessore2015a}.




We include an external shear characterized by a deflection angle, where $(x,y)$ are image coordinates:
\begin{equation}
    \alpha_{ext}(x,y)=\left(\gamma_{ext, 1}x+\gamma_{ext, 2}y, \gamma_{ext, 2}x-\gamma_{ext, 1}y\right).
\end{equation}




The elliptical \ser profile is defined as:
\begin{equation}
I(x_{light}, y_{light})= I_0 \ exp\left(-b_n\left(\left(\frac{\sqrt{q x_{light}^2+y_{light}^2 / q}}{R}\right)^{1/n} - 1
\right)
\right),
\end{equation}
where $b_n = 1.9992 n - 0.3271$, $n$ is the Sérsic index, $(x_{light}, y_{light})$ are light-centric coordinates, and $R$ is the half-light radius. 

Finally, in lens modeling, eccentricities are often used through a reparametrization,
\begin{equation}
    (\epsilon_1, \epsilon_2) = \frac{1-q}{1+q}\left(cos(2\phi), sin(2\phi)\right),
\end{equation}
where $\phi$ is the position angle. 
